Enhancing Federated Graph Learning via Adaptive Fusion of Structural and Node Characteristics

Federated Graph Learning (FGL) has demonstrated the advantage of training a global Graph Neural Network (GNN) model across distributed clients using their local graph data. Unlike Euclidean data (\eg, images), graph data is composed of nodes and edges, where the overall node-edge connections determine the topological structure, and individual nodes along with their neighbors capture local node features. However, existing studies tend to prioritize one aspect over the other, leading to an incomplete understanding of the data and the potential misidentification of key characteristics across varying graph scenarios. Additionally, the non-independent and identically distributed (non-IID) nature of graph data makes the extraction of these two data characteristics even more challenging. To address the above issues, we propose a novel FGL framework, named FedGCF, which aims to simultaneously extract and fuse structural properties and node features to effectively handle diverse graph scenarios. FedGCF first clusters clients by structural similarity, performing model aggregation within each cluster to form the shared structural model. Next, FedGCF selects the clients with common node features and aggregates their models to generate a common node model. This model is then propagated to all clients, allowing common node features to be shared. By combining these two models with a proper ratio, FedGCF can achieve a comprehensive understanding of the graph data and deliver better performance, even under non-IID distributions. Experimental results show that FedGCF improves accuracy by 4.94%-7.24% under different data distributions and reduces communication cost by 64.18%-81.25% to reach the same accuracy compared to baselines.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> papercontent/analysis.tex <==
In this section, we present the convergence analysis for our proposed scheme, and prove that the models of the edge nodes in the network converge to the same optima.
In order to prove it, we first make the following four assumptions, referring to \cite{}.

\begin{assumption}\label{assumption:lipschitzian}
    \textbf{(Lipschitzian Gradient)} Each local loss function $F(\omega_i)$ and its local gradient $\nabla F(\omega_i)$ are $L$-$Lipschitz$: $\|\nabla F(x)-\nabla F(y)\|_{2} \leq L\|x-y\|_{2},\forall x,y\in\mathcal{R}^d$.
\end{assumption}

\begin{assumption}
    \textbf{(Bounded Gradient Variance)} The variance of stochastic gradients at each worker is bounded: $\mathbb{E}\|\nabla f(\omega_{i};\xi_{i})-\nabla F(\omega_{i})\|\leq \delta^2,\forall \omega_{i}\in \mathcal{R}^d$.
\end{assumption}

\begin{assumption}\label{assumption:spectralgap}
    \textbf{(Spectral Gap)} At each epoch $t$, given the matrix $\mathbf{W}^{t}$, we define the spectral norm $\sigma=\|\mathbb{E}[(\mathbf{W}^{t})^{\mathbb{T}} \mathbf{W}^{t}]-\frac{\mathbf{1} \times \mathbf{1}^{\mathrm{T}}}{|\mathcal{M}|}\|_{2}<1$.
\end{assumption}

\begin{assumption}\label{assumption:additivenoise}
    \textbf{(Additive Noise)} For each worker $i$, its stochastic gradients have additive noise $\varepsilon_i$ which caused by stochastic sampling from the dataset. It has zero mean $\mathbb{E}[\varepsilon_i]=0$ and bounded variance $\mathbb{E}[\varepsilon_{i}^{\mathbb{T}}\varepsilon_{i}]\leq\varphi^2$.
\end{assumption} 
\begin{remark}
    Let $\mu>0$, the loss function $F$ is $\mu$-strongly convex if $\forall x,y$,
    $F(y)-F(x) \geq\langle\nabla F(x), y-x\rangle+\frac{\mu}{2}\|y-x\|^{2}$.
\end{remark}
\begin{remark}\label{lemma:1}
    Let $\mu\geq 0$ and the local loss function $F$ is $\mu$-strongly convex.
    Combining Assumption \ref{assumption:lipschitzian} and the property of convex functions, $\forall x, y\in\mathcal{R}^d$, we have 
    \begin{flalign}
        &(\nabla F(x)-\nabla F(y))^{\mathbb{T}}(x-y) \notag\\
        &\geq \frac{\mu L}{\mu+L}(x-y)^{\mathbb{T}}(x-y) \notag\\
        &\quad+\frac{1}{\mu+L}(\nabla F(x)-\nabla F(y))^{\mathbb{T}}(\nabla F(x)-\nabla F(y))
    \end{flalign}
\end{remark}
According to Alg. \ref{alg:workerprocess}, the worker updates the local model in two steps at epoch $t$.
The first update of worker $i$ using computed stochastic gradient (Line \ref{alg:line:computeend}) can be written as:
\begin{equation}\label{equ:firstupdate}
    \omega_{i}^{t+\frac{1}{2}}=\omega_{i}^{t}-\eta g_{i}^{t}
\end{equation}
For simplicity, let $\tau_{i,j}=\frac{(d_{i,j}+d_{j,i})}{4\ln p_{i,j}}$. The second update of worker $i$ using the neighbors' parameters (Line \ref{alg:line:averagebegin}-\ref{alg:line:averageend}) can be written as:
\begin{flalign}\label{equ:secondupdate}
    %\begin{split}
    \omega_{i}^{T+1}&=\omega_i^{t+\frac{1}{2}}+\eta\rho\sum_{j\in \mathcal{Z}_i}\tau_{i,j}(\omega_i^{t+\frac{1}{2}}-\omega_j^t))\notag\\
    &=\omega_i^{t}-\eta g_{i}^{t}+\eta\rho\sum_{j\in \mathcal{Z}_i}\tau_{i,j}(\omega_i^{t}-\eta g_{i}^{t}-\omega_j^t))\notag\\ 
    &=(1+\eta\rho\sum_{j\in \mathcal{Z}_i}\tau_{i,j})(\omega_i^{t}-\eta g_{i}^{t})-\eta\rho\sum_{j\in \mathcal{Z}_i}\tau_{i,j}\omega_j^{t}
    %\end{split}
\end{flalign}
% \begin{flalign}\label{equ:secondupdate}
%     %\begin{split}
%     \omega_{i}^{T+1}&=\omega_i^{t+\frac{1}{2}}-\eta\rho\sum_{j\in \mathcal{Z}_i}\tau_{i,j}(\omega_i^{t+\frac{1}{2}}-\omega_j^t))\notag\\
%     &=\omega_i^{t}-\eta g_{i}^{t}-\eta\rho\sum_{j\in \mathcal{Z}_i}\tau_{i,j}(\omega_i^{t}-\eta g_{i}^{t}-\omega_j^t))\notag\\ 
%     &=(1-\eta\rho\sum_{j\in \mathcal{Z}_i}\tau_{i,j})(\omega_i^{t}-\eta g_{i}^{t})+\eta\rho\sum_{j\in \mathcal{Z}_i}\tau_{i,j}\omega_j^{t}
%     %\end{split}
% \end{flalign}
Thus, Eq. \eqref{equ:secondupdate} can be rewritten as matrix form:
\begin{equation}\label{equ:general}
    \Omega^{t+1}=\mathbf{W}^{t}(\Omega^{t}-\eta\boldsymbol{g}^{t})
\end{equation} 
where $\Omega^{t}$ is a vector containing all workers' models and $\boldsymbol{g}^{t}$ is a vector containing all workers' gradients at epoch $t$.
$\mathbf{W}^{t}$ is an $m\times m$ matrix which can be expressed as:
\begin{equation}\label{equ:wt}
    \mathbf{W}^{t}=\boldsymbol{I}+\eta\rho\mathbf{U}
\end{equation}
where $\mathbf{U}$ is also an $m\times m$ symmetric matrix, in which the diagonal element is $\sum_{i\in\mathcal{Z}_i}\tau_{i,j},\forall i$ and non-diagonal element is $\tau_{i,j},\forall i\neq j$.
Thus, the matrix $\mathbf{W}$ is associated with the communication policy matrix $\mathbf{P}$.
By applying Eq. \eqref{equ:wt}, the expectation below is derived with respect to the matrix $\mathbf{W}$ as follows: 
% \begin{equation}
%     \mathbf{W}^{t}=\boldsymbol{I}+\eta\rho\tau_{i,j}\boldsymbol{u}_i(\boldsymbol{u}_{z}-\boldsymbol{u}_i)^{\mathbb{T}}
% \end{equation}
% where $\boldsymbol{u}_i$ is an $m\times 1$ unit vector with $i$-th component equal to 1.
% $\boldsymbol{u}_j$ is also an $m\times 1$ unit vector, where the 
\begin{flalign}
    \mathbf{Y}&=\mathbb{E}\left[(\mathbf{W}^{t})^{\mathbb{T}}\mathbf{W}^{t}\right]\notag\\
    &=\mathbb{E}\left[\boldsymbol{I}+\eta\rho\mathbf{U}^{\mathbb{T}}+\eta\rho\mathbf{U}+\eta^{2}\rho^{2}\mathbf{U}^{\mathbb{T}}\mathbf{U}\right]\\
    &=[y_{i,j}]_{m\times m}
\end{flalign}
where
\begin{equation}
    \begin{cases}
        y_{i,i}=1+2\eta\rho\sum_{j\in\mathcal{Z}_i}\tau_{i,j}p_{i,j}\\
        \quad\quad + \eta^2\rho^2\left[(\sum_{j\in\mathcal{Z}_i}\tau_{i,j})^2+\sum_{j\in\mathcal{Z}_i}p_{i,j}\tau_{i,j}p_{j,i}\tau_{j,i}\right],\forall i\in \mathcal{M}\\
        y_{i,j}=\eta\rho(p_{i,j}\tau_{i,j}+p_{j,i}\tau_{j,i})\\
        \quad\quad + \eta^2\rho^2\left[\sum_{j\in\mathcal{Z}_i}p_{i,j}\tau_{i,j}\tau_{j,i}+\sum_{k\in\mathcal{Z}_j}p_{j,k}\tau_{j,k}\tau_{k,j}\right], \forall i\neq j\\
        
    \end{cases}
\end{equation}
We use $\alpha_1$ and $\alpha_2$ to denote the largest and second largest eigenvalue of the matrix $\mathbf{Y}$, respecitively.
Let $\alpha=\alpha_2$ if $\mathbf{Y}$ is a doubly stochastic symmetric matrix; otherwise, let $\alpha=\alpha_1$.
It should be noted that there is a situation in which a worker does not communicate with any of its neighbors at an epoch, resulting in unconnected communication.
However, the model training can achieve convergence if the Assumption \ref{assumption:spectralgap} is satisfied and the undirected graph $\mathcal{G}$ connecting workers is connected \cite{}. Then we can derive the following two theorems.

\begin{theorem}
    Combining the assumptions and the lemma, when CE-DFL is performed in the form of Eq. \eqref{equ:general} with the learning rate $0<\eta\leq \frac{2}{\mu+L}$, we have
    \begin{equation}
        \mathbb{E}\left[\left\|\Omega^{T}-\omega^{*} \mathbf{1}\right\|^{2}\right]\leq\alpha^{T}\|\Omega^{0}-\omega^{*}\mathbf{1}\|^{2}+\frac{\alpha}{1-\alpha}\eta^{2}\varphi^{2}
    \end{equation}
    and CD-DFL will converge to a small domain after $T$ epochs if $\alpha<1$.
    Here $\alpha^T$ denotes the $T$-th power of $\alpha$.
\end{theorem}

\begin{proof}
    When CD-DFL has been performed $T+1$ epochs, we can derive the following equalities and inequalities by applying Eq. \eqref{equ:general}:
    \begin{flalign}\label{equ:1}
        %\begin{array}{l}
            &\mathbb{E}\left[|\Omega^{T+1}-\omega^{*} \mathbf{1}\|^{2} \right] \notag\\
            &=\mathbb{E}\left[\|\boldsymbol{W}^{T}\left(\Omega^{T}-\eta \boldsymbol{g}^{T}\right)-\omega^{*} \mathbf{1}\|^{2} \right] \notag\\
            &=\mathbb{E}\left[\left(\Omega^{T}-\omega^{*}\mathbf{1}-\eta \boldsymbol{g}^{T}\right)^{\mathbb{T}}(\boldsymbol{W}^{T})^{\mathbb{T}} \boldsymbol{W}^{T}\left(\Omega^{T}-\omega^{*}\mathbf{1}-\eta \boldsymbol{g}^{T}\right) \right] \notag\\
            &\leq \alpha \mathbb{E}\left[\left(\Omega^{T}-\omega^{*}\mathbf{1}-\eta \boldsymbol{g}^{T}\right)^{\mathbb{T}}\left(\Omega^{T}-\omega^{*}\mathbf{1}
            -\eta \boldsymbol{g}^{T}\right)\right]\notag\\
            &=\alpha\mathbb{E}\left[\left\|\Omega^{T}-\omega^{*} \mathbf{1}\right\|^{2}-2 \eta\left(\boldsymbol{g}^{T}\right)^{\mathbb{T}}\left(\Omega^{T}-\omega^{*} \mathbf{1}\right)+\eta^{2}\left(\boldsymbol{g}^{T}\right)^{\mathbb{T}} \boldsymbol{g}^{T} \right] \notag\\
        &\leq\alpha\left\|\Omega^{T}-\omega^{*} \mathbf{1}\right\|^{2}-2 \alpha\eta \sum_{i\in\mathcal{M}}  \nabla F\left(\omega_{i}^{T}\right)^{\mathbb{T}}\left(\omega_{i}^{T}-\omega^{*}\right) \notag\\
        &\quad+\alpha\eta^{2} \sum_{i\in\mathcal{M}}  \nabla F\left(\omega_{i}^{T}\right)^{\mathbb{T}} \nabla F\left(\omega_{i}^{T}\right)+\alpha\eta^{2} \sum_{i\in\mathcal{M}} \mathbb{E}\left[\left(\varepsilon_{i}^{T}\right)^{\mathbb{T}} \varepsilon_{i}^{T}\right]
            %\end{array}
    \end{flalign}
    % \begin{flalign}
    %     &\mathbb{E}\left[\left(\Omega^{T}-\omega^{*} \mathbf{1}-\eta \boldsymbol{g}^{T}\right)^{\mathbb{T}}\left(\Omega^{T}-\omega^{*}\mathbf{1}-\eta \boldsymbol{g}^{T}\right)\right] \notag\\
    %     &=\mathbb{E}\left[\left\|\Omega^{T}-\omega^{*} \mathbf{1}\right\|^{2}-2 \eta\left(\boldsymbol{g}^{T}\right)^{\mathbb{T}}\left(\Omega^{T}-\omega^{*} \mathbf{1}\right)+\eta^{2}\left(\boldsymbol{g}^{T}\right)^{\mathbb{T}} \boldsymbol{g}^{T} \right] \notag\\
    %     &=\left\|\Omega^{T}-\omega^{*} \mathbf{1}\right\|^{2}-2 \eta \sum_{i\in\mathcal{M}}  \nabla F\left(\omega_{i}^{T}\right)^{\mathbb{T}}\left(\omega_{i}^{T}-\omega^{*}\right) \notag\\
    %     &\quad+\eta^{2} \sum_{i\in\mathcal{M}}  \nabla F\left(\omega_{i}^{T}\right)^{\mathbb{T}} \nabla F\left(\omega_{i}^{T}\right)+\eta^{2} \sum_{i\in\mathcal{M}} \mathbb{E}\left[\left(\varepsilon_{i}^{T}\right)^{\mathbb{T}} \varepsilon_{i}^{T}\right]
    %     \end{flalign}
Combining the Remark \ref{lemma:1} and let $x=\omega_{i}^{T}$, $y=\omega^{*}$, we have that
        \begin{flalign}\label{equ:strongconvex}
                &-\nabla\left(F\left(\omega_{i}^{T}\right)-0\right)^{\mathbb{T}}\left(\omega_{i}^{T}-\omega^{*}\right)= -\nabla F\left(\omega_{i}^{T}\right)^{\mathbb{T}}\left(\omega_{i}^{T}-\omega^{*}\right)\notag\\
                &\leq-\frac{\mu L}{\mu+L}\left(\omega_{i}^{T}-\omega^{*}\right)^{\mathbb{T}}\left(\omega_{i}^{T}-\omega^{*}\right)\notag\\
                &\qquad-\frac{1}{\mu+L} \nabla F\left(\omega_{i}^{T}\right)^{\mathbb{T}} \nabla F\left(\omega_{i}^{T}\right)
        \end{flalign}

        By applying Eq. \eqref{equ:strongconvex} into the second term of the last inequality in Eq. \eqref{equ:1}, we can bound
        s
        \begin{flalign}\label{equ:2}
                - &2 \alpha\eta \sum_{i\in\mathcal{M}} \nabla F\left(\omega_{i}^{T}\right)^{\mathbb{T}}\left(\omega_{i}^{T}-\omega^{*}\right) \notag\\
                \leq&-\frac{2 \alpha\eta \mu L}{\mu+L} \sum_{i\in\mathcal{M}} \left(\omega_{i}^{T}-\omega^{*}\right)^{\mathbb{T}}\left(\omega_{i}^{T}-\omega^{*}\right) \notag\\
                &-\frac{2 \alpha\eta}{\mu+L} \sum_{i\in\mathcal{M}} \nabla F\left(\omega_{i}^{T}\right)^{\mathbb{T}} \nabla F\left(\omega_{i}^{T}\right) 
                % \leq& -\frac{2 \eta \mu L}{\mu+L} p_{\min } \sum_{n=1}^{M}\left(\Omega_{i}^{t}-\omega^{*}\right)^{\mathbb{T}}\left(\Omega_{i}^{t}-\omega^{*}\right) \notag\\
                % &-\frac{2 \eta}{\mu+L} \sum_{n=1}^{M} p_{n} \nabla f\left(\Omega_{i}^{t}\right)^{\mathbb{T}} \nabla f\left(\Omega_{i}^{t}\right)
        \end{flalign}

        Combining Eq. \eqref{equ:1} and Eq. \eqref{equ:2}, we have that

        \begin{flalign}\label{equ:3}
            &\mathbb{E}\left[\left\|\Omega^{T+1}-\omega^{*} \mathbf{1}\right\|^{2} \right] \notag\\
            &\leq \alpha \mathbb{E}\left[\left(\Omega^{T}-\omega^{*} \mathbf{1}-\eta \boldsymbol{g}^{T}\right)^{\mathbb{T}}\left(\Omega^{T}-\omega^{*} \mathbf{1}-\eta \boldsymbol{g}^{T}\right) \right] \notag\\
            &\leq\alpha\left(1-\frac{2 \eta \mu L}{\mu+L}\right)\left\|\Omega^{T}-\omega^{*} \mathbf{1}\right\|^{2}+\alpha\eta^{2} \varphi^{2} \notag\\
            &\quad+\alpha\left(\eta^{2}-\frac{2 \eta}{\mu+L}\right) \sum_{i\in\mathcal{M}} \nabla F\left(\omega_{i}^{T}\right)^{\mathbb{T}} \nabla F\left(\omega_{i}^{T}\right)\notag\\
            % &\leq\left(1-\frac{2 \eta \mu L}{\mu+L} \right)\left\|\Omega^{T}-\omega^{*} \mathbf{1}\right\|^{2}+\eta^{2} \varphi^{2}\\
            &\leq \alpha\left(1-\frac{2 \eta \mu L}{\mu+L} \right)\left\|\Omega^{T}-\omega^{*} \mathbf{1}\right\|^{2}+\alpha \eta^{2} \varphi^{2} \notag\\
            &\leq \alpha\left\|\Omega^{T}-\omega^{*} \mathbf{1}\right\|^{2}+\alpha \eta^{2} \varphi^{2}
    \end{flalign}
        % \begin{flalign}
        %         &\mathbb{E}\left[\left(\Omega^{T}-\omega^{*} \mathbf{1}-\eta \boldsymbol{g}^{T}\right)^{\mathbb{T}}\left(\Omega^{T}-\omega^{*} \mathbf{1}-\eta \boldsymbol{g}^{T}\right) \right] \notag\\
        %         &\leq\left(1-\frac{2 \eta \mu L}{\mu+L}\right)\left\|\Omega^{T}-\omega^{*} \mathbf{1}\right\|^{2}+\eta^{2} \varphi^{2} \notag\\
        %         &\quad+\left(\eta^{2}-\frac{2 \eta}{\mu+L}\right) \sum_{i\in\mathcal{M}} \nabla F\left(\omega_{i}^{T}\right)^{\mathbb{T}} \nabla F\left(\omega_{i}^{T}\right)\notag\\
        %         &\leq\left(1-\frac{2 \eta \mu L}{\mu+L} \right)\left\|\Omega^{T}-\omega^{*} \mathbf{1}\right\|^{2}+\eta^{2} \varphi^{2}
        % \end{flalign}

        % \begin{flalign}
        %         &\mathbb{E}\left[\left\|\Omega^{T+1}-\omega^{*} \mathbf{1}\right\|^{2} \right] \notag\\
                
        %         &\leq \alpha \mathbb{E}\left[\left(\Omega^{T}-\omega^{*} \mathbf{1}-\eta \boldsymbol{g}^{T}\right)^{\mathbb{T}}\left(\Omega^{T}-\omega^{*} \mathbf{1}-\eta \boldsymbol{g}^{T}\right) \right] \notag\\
        %         &\leq \alpha\left(1-\frac{2 \eta \mu L}{\mu+L} \right)\left\|\Omega^{T}-\omega^{*} \mathbf{1}\right\|^{2}+\alpha \eta^{2} \varphi^{2} \notag\\
        %         &\leq \alpha\left\|\Omega^{T}-\omega^{*} \mathbf{1}\right\|^{2}+\alpha \eta^{2} \varphi^{2}
        % \end{flalign}

    Finally, the convergence bound after $T$ training epochs can be
    derived as follows

        \begin{flalign}
            &\mathbb{E}\left[\left\|\Omega^{T}-\omega^{*} \mathbf{1}\right\|^{2}\right]\notag\\ 
            &\leq\alpha\left\|\Omega^{T-1}-\omega^{*} \mathbf{1}\right\|^{2}+\alpha \eta^{2} \varphi^{2} \notag\\ 
            &......\qquad(\text{Telescoping by Eq. \eqref{equ:3}}) \notag\\
            &\leq\alpha^{T}\left\|\Omega^{0}-\omega^{*} \mathbf{1}\right\|^{2}+\frac{1-\alpha^T}{1-\alpha}\alpha \eta^{2} \varphi^{2} \notag\\
            &\leq\alpha^{T}\left\|\Omega^{0}-\omega^{*} \mathbf{1}\right\|^{2}+\frac{\alpha}{1-\alpha} \eta^{2} \varphi^{2}
        \end{flalign}

\end{proof}

% 





==> papercontent/convergence.tex <==
%\section{convergence Analysis}\label{sec:convergence analysis}
In this section, we analyze the convergence property of the proposed FedACS approximately. We rewrite the global model $\omega_{t}$ update function in Eq. (\ref{Agg}) as follows:
\begin{equation}
	\omega_{t+1}=\sum_{i \in V_{t}}\frac{n_i}{n'}\omega_{t,i}=\sum_{i \in V_{t}}\frac{n_i}{n'}(\omega_{t}-\eta \nabla F_i(\omega_{t,i};H_{t,i}))
\end{equation}
%We define $H_{t,i}=(x_{t,k}, e_{t,k}, l_{k})$ and $\nabla F_k(\omega_{t,k},H_{t,k})=\frac{1}{n^k}\sum_{h_{t,k} \in H_{t,k}}\nabla F_k(\omega_{t,k},h_{t,k})$, the above denotes global parameter updata.%
We define $H_{t,i}=(x_{i,u}, x_{i,v}, z_{u,v}), u,v\in V_{i}, v\in\mathcal{N}_u$, as a mini-batch of samples graph data $d_i$. $n_i$ represents the size of data samples while $\mathcal{N}_u$ is the neighbor set of node $u$. Let $\nabla F_i(\omega_{t,i};H_{t,i})=\frac{1}{n_i}\sum_{h_{t,i} \in H_{t,i}}\nabla f(\omega_{t,i},h_{t,i})$, $f$ is the loss function of the global GNN model with $h_{t,i}$ data samples.
To analyze the convergence of FedACS, we assume that our problem satisfies the following assumptions, which have been adopted in previous works \cite{convergence} on the convergence analysis.

\begin{assumption}
	Each function $F_i(\omega,H_{t,i}),\forall i \in [N]$, has an $L$-lipschitz gradient with respect to $\omega$, and $\nabla_wF_i(\omega,H_{t,i})$ is $L_{e}$-lipschitz with respect to $H_{t,i}$.
\end{assumption}

\begin{assumption}
	All neighbors of a node are used for embedding generation, the gradient computed using the mini-batches w.r.t $\omega$ is an unbiased estimator of the true gradient and has a bounded variance at each client $i$. That is, $\mathbb{E}[\nabla F_{i}(\omega, H_{t,i})] = \nabla F_{i}(\omega, \mathcal{V}_i)$, $\mathbb{E}[\|\nabla F_i(\omega,H_{t,i})-\nabla F_k(\omega,\mathcal{V}_i)\|^2]\leq \delta^2,\forall i$.
\end{assumption}
%
%\begin{assumption}
%The parameter synchronization interval satisfies $E=K\tau$.
%\end{assumption}
%

%\begin{assumption}
%	The expected gradient norm of full neighbour set training across all clients is upper bounded by the norm of expected gradient of neighbour set training in subgraph for all clients:$\sum_{i \in C}\frac{n_i}{n}\mathbb{E}[\|\nabla F_i(\omega_{t,i}, h_{t,i})\|^2] \leq \beta \mathbb{E}[\|\sum_{i \in C}\frac{n^k}{n}\nabla F_i(\omega_{t,i}, hs_{t,i})\|^2]$.
%\end{assumption}

\begin{assumption}
	The loss function values of the train data and the test data are positively correlated for each client. Clients $c_{t}$ selected based on test data scores also have higher loss function values than the other clients. That is, $\sum_{i \in V_{t}}\frac{n_i}{n'}\nabla F_i(\omega_{t,i},H_{t,i}) \geq \sum_{i=1}^{N}\frac{n_{i}}{n}\nabla F_i(\omega_{t,i},H_{t,i})  $
\end{assumption}

To facilitate convergence analysis, we use an intermediate variable $\bar{\omega}_t = \sum_{i \in V_{t}}\frac{n_i}{n'}\omega_{t,i}$. So we have $\bar{\omega}_{t+1}=\bar{\omega}_t-\eta \sum_{i \in V_{t}} \frac{n_i}{n'}\nabla F_i(\omega_{t},H_{t,i})$. We use the expected gradient norm as the convergence metric that follows the convention in non-convex optimization \cite{convergence}.

Based on Assumption 1, we have
\begin{equation}
	\begin{split}
		\mathbb{E}[F(\bar{\omega}_{t+1})]& \leq \mathbb{E}[F(\bar{\omega}_{t})]+\mathbb{E}[\langle \nabla F(\bar{\omega}_t),\bar{\omega}_{t+1}-\bar{\omega}_t\rangle]\\
		& +\frac{L}{2}\mathbb{E}[\|\bar{\omega}_{t+1}-\bar{\omega}_{t}\|^2]
	\end{split}
\end{equation}
To enhance the understanding of the convergence analysis, let $d_t = \sum_{i=1}^{N}\frac{n_{i}}{n}\nabla F_i(\omega_{t,i},H_{t,i})$. And according to the inner product formula $\langle a,b\rangle=\frac{1}{2}\|a\|^2+\frac{1}{2}\|b\|^2-\frac{1}{2}\|a-b\|^2$ and  the norm inequality $\|a+b\|^2\leq2(\|a\|^2+\|b\|^2)$, we have the following result:
\begin{equation}\label{ccc}
	\begin{split}
		\mathbb{E}[F(\bar{\omega}_{t+1})] & \leq \mathbb{E}[F(\bar{\omega}_{t})]+(L\eta^2-\frac{\eta}{2})\mathbb{E}[\|\nabla F(\bar{\omega}_t)\|^2]\\
		& -\frac{\eta}{2}\mathbb{E}[\|d_t\|^2]+(L\eta^2+\frac{\eta}{2})\mathbb{E}[\|\nabla F(\bar{\omega}_t)-d_t\|^2]
	\end{split}
\end{equation}


Next, we discuss the upper bound of $\mathbb{E}[\|\nabla F(\bar{\omega}_t)-d_t\|^2]$. According to previous work \cite{convergence}, we have the following lemma:
\begin{lemma}\label{lemma}
	\begin{equation}
		%\begin{split}
			\mathbb{E}[\|\nabla F(\bar{\omega}_t)-d_t\|^2]
			 \leq 3[\delta^2 +2L^2\eta^2\sum_{i \in N}\frac{n_i}{n}\mathbb{E}[\|\nabla F_i(\omega_{t},H_{t,i})\|^2]]
		%\end{split}
	\end{equation}
\end{lemma}
According to Eq. \eqref{ccc}, we have the following:
\begin{equation}\label{ddd}
	\begin{split}
		&(\frac{\eta}{2}-L\eta^2)\mathbb{E}[\|\nabla F(\bar{\omega}_t)\|^2] \leq (\mathbb{E}[F(\bar{\omega}_{t})]-\mathbb{E}[F(\bar{\omega}_{t+1})])\\
		&-\frac{\eta}{2}\mathbb{E}[\|d_t\|^2]+(L\eta^2+\frac{\eta}{2})\mathbb{E}[\|\nabla F(\bar{\omega}_t)-d_t\|^2]
	\end{split}
\end{equation}
We use $F'$ and $T$ to denote the optimal value of function $F$ and the number of total round, respectively. We incorporate the findings derived from Lemma \ref{lemma} into Eq. \eqref{ddd} for further analysis:
\begin{equation}
	\begin{split}
		&(\frac{\eta}{2}-L\eta^2)\frac{\sum_{t=1}^{T}\mathbb{E}[\|\nabla F(\bar{\omega}_t)\|^2]}{T}\\
		&\leq\frac{F(\bar{\omega}_1)-F'}{T}-\frac{\eta}{2}\frac{\sum_{t=1}^{T}\mathbb{E}[d_t]}{T}+3(L\eta^2+\frac{\eta}{2})\\
		&(\delta^2+2L^2\eta^2\frac{\sum_{t=1}^{T}\mathbb{E}[\|d_t\|^2]}{T})
	\end{split}
\end{equation}

%Next, we discuss the value of learning rate $\eta$. First, we want $(\frac{\eta}{2}-L\eta^2)\geq0, \eta\leq\frac{1}{2L}$. Let $3(L\eta^2+\frac{\eta}{2})2L^2\eta^2\leq\frac{\eta}{2}$ to remove $\frac{\sum_{t=1}^{T}\mathbb{E}[\|d_t\|^2]}{T}$, which would be equivalent to solving $3(L\eta+\frac{1}{2})2L^2\eta^2-\frac{1}{2} \leq 0$. Taking the derivation of $\eta$, we have $2L^2\eta(9L\eta+1)$ and the result is non-negative when $\eta\geq0$. When $\eta=0$, the result would be $-\frac{1}{2}$. Therefore, there must be $\eta\ge0$ making the inequality establish. We use $\bar{\eta}$ to denote the maximum value of $\eta$ which holds the inequality.
Next, we discuss the value of learning rate $\eta$. First, in order to ensure the convergence of the formula, we set the condition: $(\frac{\eta}{2}-L\eta^2)\geq0, \eta\leq\frac{1}{2L}$. Next, to simplify the above result, we introduce another condition to eliminate the term: $\frac{\sum_{t=1}^{T}\mathbb{E}[\|d_t\|^2]}{T}$. This is achieved by setting: $3(L\eta^2+\frac{\eta}{2})2L^2\eta^2\leq\frac{\eta}{2}$, which would be equivalent to solving the inequality $3(L\eta+\frac{1}{2})2L^2\eta^2-\frac{1}{2} \leq 0$. Upon differentiating this inequality with respect to $\eta$, we have $2L^2\eta(9L\eta+1)$. This derivative is non-negative for all $\eta\geq0$. When $\eta=0$, the result would be $-\frac{1}{2}$. Therefore, there must be $\eta\ge0$ to make the inequality establish. We use $\bar{\eta}$ to denote the maximum value of $\eta$ which holds the inequality.

To sum up, when the learning rate $\eta\leq min \{\frac{1}{2L},\bar{\eta}\}$, we have
\begin{equation}
	\begin{split}
		&\frac{\sum_{t=1}^{T}\mathbb{E}[\|\nabla F(\bar{\omega}_t)\|^2]}{T}\leq\frac{F(\bar{\omega}_1)-F'}{T(\frac{\eta}{2}-L\eta^2)}
		+3\frac{(L\eta^2+\frac{\eta}{2})}{(\frac{\eta}{2}-L\eta^2)}\delta^2
	\end{split}
\end{equation}

% The similar proof of lemma \ref{lemma} can be found in previous work \cite{convergence}.

==> papercontent/implement.tex <==
\section{Implement} \label{sub:implement}
\begin{table*}[htbp]
	\centering
	%\vspace{-0.05cm}
	\renewcommand{\arraystretch}{1.1}
	\hspace{3mm}
	\caption{Overall scores performance}\label{overall performance}
	\setlength{\abovecaptionskip}{10pt}%
	\setlength{\belowcaptionskip}{10pt}%
	\footnotesize
	\small
	\centering
	\begin{tabular}{c|ccc|ccc}
		\hline
		% \multirow{2}{*}{Name}，2为所占的行数，此语句可以使得内容垂直居中
		% \multicolumn{2}{c|}{Flag}，2为所占的列数，格式由第二个{}控制
		% \cline{2-3}指本行的2,3列画横线
        \multirow{2}{*}{Mehtod} & \multicolumn{3}{c|}{Ciao} &\multicolumn{3}{c}{Epinions}\\\cline{2-7} 
        &MAE   & RMSE &  MSE &MAE   & RMSE &  MSE \\\hline
		SoRec &0.943 &1.252 &1.569 &1.014 &1.482 &2.198\\
		SoReg &0.929 &1.233 &1.519 &1.013 &1.480 &2.193\\
		Consisrec &0.734 &0.978 &0.956 &0.829 &1.062 &1.127\\\hline
		FedGNN &2.008 &2.528 &6.393 &2.902 &3.250 &10.562\\\
		FedSoG &1.578 &2.062 &4.251 &1.426 &1.833 &3.361\\\
		FedGraphNN (GAT model) &0.804 &1.054 &1.121 &1.051 &1.219 &1.489\\\
		FedGraphNN (GCN model) &0.810 &1.053 &1.121 &0.955 &1.196 &1.433\\\hline
		FedACS (GAT model)&\textbf{0.803} &\textbf{1.039} &\textbf{1.091} &0.918 &\textbf{1.168} &\textbf{1.370}\\\
		FedACS (GCN model)&0.804 &1.039 &1.091 &\textbf{0.910} &1.170 &1.373\\\hline
	\end{tabular}
        \label{TABLE_a}
\end{table*}

\begin{table*}[t]
	\centering
	%\vspace{-0.05cm}
	\renewcommand{\arraystretch}{1.1}
	\hspace{3mm}
	\caption{Resources performance}\label{overall performance}
	\setlength{\abovecaptionskip}{10pt}%
	\setlength{\belowcaptionskip}{10pt}%
	\footnotesize
	\small
	\centering
	\begin{tabular}{c|ccc|ccc}
		\hline
		% \multirow{2}{*}{Name}，2为所占的行数，此语句可以使得内容垂直居中
		% \multicolumn{2}{c|}{Flag}，2为所占的列数，格式由第二个{}控制
		% \cline{2-3}指本行的2,3列画横线
		\multirow{2}{*}{Mehtod} & \multicolumn{3}{c|}{Ciao} &\multicolumn{3}{c}{Epinions}\\\cline{2-7}
		& RMSE &Communication resource (KB)   & Time (s) &RMSE &Communication resource (KB)   & Time (s) \\\hline
            FedGNN &2.528 &9996 &6003 &3.250 &9996 &15599\\\
		FedSoG &2.062 &21990 &12537 &1.833 &21990 &32775\\\
		FedGraphNN (GAT model) &1.055 &851 &90 &1.219 &851 &382\\\
		FedGraphNN  (GCN model) &1.052 &851 &119 &1.196 &851 &538\\\hline
            FedACS (GAT model) &1.039 &\textbf{332} &\textbf{75} &\textbf{1.168} &\textbf{447} &\textbf{326}\\\
		FedACS (GCN model) &\textbf{1.039} &568 &98 &1.170 &476 &406\\\hline
	\end{tabular}
        \label{TABLE_b}
\end{table*}

\begin{table*}[t]
	\centering
	%\vspace{-0.05cm}
	\renewcommand{\arraystretch}{1.1}
	\hspace{3mm}
	\caption{Resources performance}\label{overall performance}
	\setlength{\abovecaptionskip}{10pt}%
	\setlength{\belowcaptionskip}{10pt}%
	\footnotesize
	\small
	\centering
	\begin{tabular}{c|ccc|ccc}
		\hline
		% \multirow{2}{*}{Name}，2为所占的行数，此语句可以使得内容垂直居中
		% \multicolumn{2}{c|}{Flag}，2为所占的列数，格式由第二个{}控制
		% \cline{2-3}指本行的2,3列画横线
		\multirow{2}{*}{Mehtod} & \multicolumn{3}{c|}{Ciao} &\multicolumn{3}{c}{Epinions}\\\cline{2-7}
		& Average & Skewed & Extreme & Average & Skewed & Extreme\\\hline
		FedGraphNN (GAT model) &1.055 &1.067 &1.038 &1.219 &1.222 &1.190\\\
		FedGraphNN  (GCN model) &1.052 &1.071 &1.041 &1.196 &1.211 &1.190\\\hline
            FedACS (GAT model) &1.039 &1.054 &1.023 &1.168 &1.166 &1.138\\\
		FedACS (GCN model) &1.039 &1.055 &1.020 &1.170 &1.170 &1.150\\\hline
	\end{tabular}
        \label{TABLE_c}
\end{table*}

\begin{table}[t]
	\centering
	%\vspace{-0.05cm}
	\renewcommand{\arraystretch}{1.1}
	\hspace{3mm}
	\caption{Resources performance}\label{overall performance}
	\setlength{\abovecaptionskip}{10pt}%
	\setlength{\belowcaptionskip}{10pt}%
	\footnotesize
	\small
	\centering
	\begin{tabular}{c|ccc}
		\hline
		% \multirow{2}{*}{Name}，2为所占的行数，此语句可以使得内容垂直居中
		% \multicolumn{2}{c|}{Flag}，2为所占的列数，格式由第二个{}控制
		% \cline{2-3}指本行的2,3列画横线
		\multirow{2}{*}{Mehtod} & \multicolumn{3}{c}{Ciao}\\\cline{2-4}
		& Average & Skewed & Extreme\\\hline
		FedGraphNN (GAT model) &1.055 &1.067 &1.038\\\
		FedGraphNN  (GCN model) &1.052 &1.071 &1.041\\\hline
            FedACS (GAT model) &1.039 &1.054 &1.023\\\
		FedACS (GCN model) &1.039 &1.055 &1.020\\\hline
	\end{tabular}
        \label{TABLE_c}
\end{table}

\begin{table}[t]
	\centering
	%\vspace{-0.05cm}
	\renewcommand{\arraystretch}{1.1}
	\hspace{3mm}
	\caption{Resources performance}\label{overall performance}
	\setlength{\abovecaptionskip}{10pt}%
	\setlength{\belowcaptionskip}{10pt}%
	\footnotesize
	\small
	\centering
	\begin{tabular}{c|ccc}
		\hline
		% \multirow{2}{*}{Name}，2为所占的行数，此语句可以使得内容垂直居中
		% \multicolumn{2}{c|}{Flag}，2为所占的列数，格式由第二个{}控制
		% \cline{2-3}指本行的2,3列画横线
		\multirow{2}{*}{Mehtod} &\multicolumn{3}{c}{Epinions}\\\cline{2-4}
		& Average & Skewed & Extreme\\\hline
		FedGraphNN (GAT model) &1.219 &1.222 &1.190\\\
		FedGraphNN  (GCN model) &1.196 &1.211 &1.190\\\hline
            FedACS (GAT model) &1.168 &1.166 &1.138\\\
		FedACS (GCN model) &1.170 &1.170 &1.150\\\hline
	\end{tabular}
        \label{TABLE_c}
\end{table}

==> papercontent/related.tex <==
%Communication bottleneck and the non-IID problem have long been plaguing problems for FGL, and existing solutions can be roughly summarized from two perspectives: one by reducing communication frequency, and the other by reducing the number of communication parameters. Some works have proposed solutions to reduce communication cost by reducing communication frequency. Zhang \etal\cite{zhang2023glasu} propose to adopt a client's up-to-date node representations and other clients' stale node representations to perform model updates in every round. As a result, the client and PS only need to communicate once every specified number of rounds. Yao \etal\cite{fedgcnfreedicide} argue that information needed to train a GCN model only needs to be shared only once before training, thus alleviating communication pressure. There are also some works making effects to reduce the communication cost by reducing the number of communication parameters. For example, Wu \etal\cite{fedgnn} and Lie \etal\cite{FeSog} all propose to upload the local gradients of GNN to a server for aggregation. Wu \etal design a novel federated framework named FedGNN, which collectively trains GNN models from decentralized user data and only uploads the local gradients of GNN to a server for aggregation. While Lie \etal adopt relational attention and aggregation to handle graph data. However, when the data distribution on the clients is non-IID, these approaches might lead to significant performance degradation. Because the stale node representations involve in the model updates and the total different neighboring node information in each client is difficult to provide help.

%To address the non-IID problem, some studies have also made efforts. Xie \etal\cite{noniid2} dynamically cluster the clients with similar data distributions based on the gradients of GNN, alleviating the non-IID problem. Tan \etal\cite{noniid1} propose to share the underlying structure information of graph data and capture more structure-based information by structure embeddings. However, these approaches require the participation of all clients, resulting in significant communication cost.

Recently, federated graph learning (FGL) has emerged, enabling collaborative training across multiple edge clients with the help of PS. A related research area to FGL focuses on communication resource efficiency due to the increasing communication demand and limited network bandwidth. Ghari \etal \cite{Graph-assisted} propose a framework to learn a set of pre-trained models. At each round, PS selects a subset of pre-trained models based on the structure of a graph and only distributes the model that satisfies the resource constraints to clients. %Zhang \etal\cite{zhang2023glasu} propose to adopt a client's up-to-date node representations and other clients' stale node representations to perform model updates in every round. 
Pan \etal \cite{fedwalk} propose to adopt a hierarchical clustering tree constructor to extract the feature of each node and use a random walk generator to update the node's embedding. While the above works mainly focus on the communication efficiency of FGL, in scenarios where the data distribution of client is non-IID, these approaches might lead to significant performance degradation.

To address the non-IID problem, some studies have made efforts. Zhang \etal  \cite{NonIID3} generate graph embeddings from the client's local graph dataset and integrate information from other clients. They also adopt the embedding alignment technique to convert the latent representations from other clients into a form that the local client can understand.
Xie \etal\cite{noniid2} theoretically justify that the heterogeneity among graphs can be reduced by dynamically finding clusters of local systems based on the gradients of the GNN model. %Xie \etal\cite{noniid2} propose a framework to dynamically find clusters of local systems based on the gradients of GNNs. 
However, these approaches require the active participation of all clients, resulting in significant communication cost. Despite the advances and extensive research endeavors in the realm of FGL, the current research has yet to fully tackle the aforementioned challenges in FGL. 
To this end, we propose FedACS, which can reduce the communication cost and alleviate the non-IID problem simultaneously.
%Wu \etal\cite{noniid4} propose to alleviate the non-IID problem by transfer learning. They design a novel graph subtree discrepancy to measure the graph distribution shift between different graphs, and minimize the distribution shift between source and target graphs for cross-network transfer learning.
%extract and share the common underlying structure information, which is encoded along with node features to enhance the local performance of clients. 
